The Hubble Space Telescope UV Legacy Survey of Galactic Globular Clusters. XVI. The helium abundance of multiple populations

Recent work, based on data from the Hubble Space Telescope (HST) UV Legacy Survey of Galactic Globular Clusters (GCs), has revealed that all the analyzed clusters host two groups of first- (1G) and second-generation (2G) stars. In most GCs, both 1G and 2G stars host sub-stellar populations with different chemical composition. We compare multi-wavelength HST photometry with synthetic spectra to determine for the first time the average helium difference between the 2G and 1G stars in a large sample of 57 GCs and the maximum helium variation within each of them. We find that in all clusters 2G stars are consistent with being enhanced in helium with respect to 1G. The maximum helium variation ranges from less than 0.01 to more than 0.10 in helium mass fraction and correlates with both the cluster mass and the color extension of the horizontal branch (HB). These findings demonstrate that the internal helium variation is one of the main (second) parameters governing the HB morphology.

==> tabella1.tex <==
\onecolumn
\begin{longtable}{lcccccccl}
\caption{Abundance difference between 2G and 1G stars and between 2Ge and 1Ge stars adopted to infer  $\delta Y_{\rm max}$ and $\delta Y_{\rm 2G,1G}$. For the clusters without literature determination of Mg, Al, and Si we adopted two sets of abundance differences corresponding to different choices of $\Delta$[Mg/Fe], $\Delta$[Al/Fe] and $\Delta$[Si/Fe]. {\bf Aggiungere referenze}}\label{tab:CNO} \\ %\hline\hline
ID        &  $\Delta$[C/Fe]     &   $\Delta$[N/Fe]  &   $\Delta$[O/Fe]  &   $\Delta$[Mg/Fe]  &   $\Delta$[Al/Fe]    &   $\Delta$[Si/Fe]  & Reference\\
\hline
\endfirsthead
\caption{continued.}\\\hline\hline
ID        &  $\Delta$[C/Fe]     &   $\Delta$[N/Fe]  &   $\Delta$[O/Fe]  &   $\Delta$[Mg/Fe]  &   $\Delta$[Al/Fe]    &   $\Delta$[Si/Fe]  & Reference \\
\hline
\endhead
\endfoot
          &                    &                    & 2G-1G&            &                  &                    &              &   \\
\hline
IC\,4499  & $-$0.05            &  0.65              & $-$0.20           &   0.00           &   0.00             &    0.00      &  --  \\
          & $-$0.05            &  0.60              & $-$0.00           &$-$0.10           &   0.80             &    0.05      &  --  \\
NGC\,104  & $-$0.30            &  0.70              & $-$0.30           &                  &                    &              &   \\
NGC\,288  & $-$0.20            &  0.70              & $-$0.65           &                  &                    &              &   \\
NGC\,362  & $-$0.25            &  0.85              & $-$0.40           &                  &                    &              &    \\
NGC\,1261 & $-$0.25            &  0.75              & $-$               &   0.00           &   0.00             &    0.00      &  --  \\
          & $-$0.45            &  0.85              & $-$               &$-$0.10           &   0.80             &    0.05      &  --  \\
NGC\,1851 & $-$0.25            &  0.85              & $-$0.35           &   0.00           &   0.40             &    0.00      &    \\
NGC\,2298 & $-$0.30            &  0.75              & $-$0.80           &   0.00           &   0.00             &    0.00      &    \\
          & $-$0.15            &  0.75              & $-$0.70           &$-$0.10           &   0.80             &    0.05      &    \\
NGC\,3201 &                    &                    &                   &                  &                    &              &    \\
NGC\,4833 & $-$0.10            &  0.85              & $-$0.30           &$-$0.15           &   0.50             &    0.05      &    \\ %
NGC\,5024 & $-$0.05            &  0.65              & $-$0.45           &   0.00           &   0.50             &    0.00      &    \\ %
NGC\,5053 &    0.20            &  0.50              &    0.00           &$-$0.10           &   1.00             &    0.10      &    \\ %
NGC\,5272 & $-$0.15            &  0.70              & $-$0.25           &$-$0.05           &   0.50             &    0.10      &  Sneden et al.\,(2004)  \\ %
NGC\,5286 & $-$0.25            &  0.90              & $-$0.55           &   0.00           &   0.00             &    0.00      &    \\ %
          & $-$0.25            &  0.80              & $-$0.20           &$-$0.10           &   0.80             &    0.05      &    \\ %
NGC\,5466 & $-$0.15            &  0.45              & $-$0.35           &   0.00           &   0.50             &    0.00      &    \\ %
NGC\,5904 & $-$0.20            &  0.80              & $-$0.35           &$-$0.05           &   0.55             &    0.00      &    \\ %
NGC\,5927 & $-$0.25            &  0.30              & $-$0.10           &  0.00            &   0.10             &    0.00      &  Pancino et al.\,(2017)  \\ %
NGC\,5986 & $-$0.25            &  0.80              & $-$0.40           &$-$0.15           &   0.50             &    0.00      &    \\ %
NGC\,6093 &    0.00            &  0.75              & $-$0.20           &   0.00           &   0.50             &    0.00      &    \\ %
NGC\,6101 & $-$0.25            &  0.85              & $-$0.60           &   0.00           &   0.00             &    0.00      &    \\ %
          & $-$0.25            &  0.70              & $-$0.25           &$-$0.10           &   0.80             &    0.05      &    \\ %
NGC\,6121 & $-$0.15            &  0.70              & $-$0.10           &   0.00           &   0.00             &    0.00      &  Marino et al.\,(2008)  \\ %
NGC\,6144 &    0.00            &  0.75              & $-$0.30           &   0.00           &   0.00             &    0.00      &    \\ %
          & $-$0.00            &  0.70              & $-$0.05           &$-$0.10           &   0.80             &    0.05      &    \\ %
NGC\,6171 & $-$0.20            &  0.60              & $-$0.10           &   0.00           &   0.00             &    0.00      &  M{\'e}sz{\'a}ros et al.(2015)  \\ %
NGC\,6205 & $-$0.15            &  0.75              & $-$0.35           &$-$0.10           &   0.80             &    0.00      &    \\ %
NGC\,6218 & $-$0.10            &  0.70              & $-$0.20           &   0.00           &   0.30             &    0.00      &    \\ %
NGC\,6254 & $-$0.30            &  0.95              & $-$0.55           &   0.00           &   0.60             &    0.00      &    \\ %
NGC\,6304 & $-$0.50            &  0.55              & $-$0.25           &   0.00           &   0.00             &    0.00      &  --  \\ %
          & $-$0.55            &  0.55              & $-$0.20           &$-$0.10           &   0.80             &    0.05      &  --  \\ %
NGC\,6341 & $-$0.40            &  0.70              & $-$0.45           &$-$0.15           &   0.75             &    0.00      &    \\ %
NGC\,6352 & $-$0.50            &  0.60              & $-$0.20           &   0.00           &   0.00             &    0.00      &  --  \\ %
          & $-$0.45            &  0.65              & $-$0.15           &$-$0.10           &   0.80             &    0.05      &  --  \\ %
NGC\,6362 & $-$0.35            &  0.70              & $-$0.30           &$-$0.00           &   0.00             &    0.00      & Massari et al.\,(2017)   \\ %
NGC\,6366 & $-$0.35            &  0.50              & $-$0.15           &$-$0.05           &   0.10             &    0.05      & Johnson et al.\,(2016); Puls et al.\,(2018)   \\ %
NGC\,6397 & $-$0.20            &  0.65              & $-$0.25           &   0.00           &   0.00             &    0.00      &    \\ %
NGC\,6441 & $-$0.70            &  0.70              & $-$0.30           &   0.10           &   0.30             &    0.10      &  Gratton et al.\,(2006); Carretta et al.\,(2009)  \\ %
NGC\,6496 & $-$0.35            &  0.45              & $-$0.15           &   0.00           &   0.00             &    0.00      &  --  \\ %
          & $-$0.35            &  0.50              & $-$0.10           &$-$0.10           &   0.80             &    0.05      &  --  \\ %
NGC\,6535 & $-$0.15            &  0.75              & $-$0.40           &   0.00           &   0.40             &    0.00      &    \\ %
NGC\,6541 & $-$0.25            &  1.00              & $-$0.75           &   0.00           &   0.00             &    0.00      &  --  \\ %
          & $-$0.20            &  0.90              & $-$0.50           &$-$0.10           &   0.80             &    0.05      &  --  \\ %
NGC\,6584 & $-$0.10            &  0.70              & $-$0.05           &   0.00           &   0.00             &    0.00      &  --  \\ %
          & $-$0.05            &  0.65              &    0.10           &$-$0.10           &   0.80             &    0.05      &  --  \\ %
NGC\,6624 & $-$0.60            &  0.60              & $-$0.40           &   0.00           &   0.00             &    0.00      &   -- \\
          & $-$0.65            &  0.65              & $-$0.35           &$-$0.10           &   0.80             &    0.05      &   -- \\ %
NGC\,6637 & $-$0.30            &  0.65              & $-$0.20           &   0.00           &   0.00             &    0.00      &   -- \\
          & $-$0.30            &  0.65              & $-$0.10           &$-$0.10           &   0.80             &    0.05      &   -- \\ %
NGC\,6652 & $-$0.30            &  0.65              & $-$0.15           &   0.00           &   0.00             &    0.00      &   -- \\
          & $-$0.25            &  0.65              & $-$0.05           &$-$0.10           &   0.80             &    0.05      &   -- \\ %
NGC\,6656 & $-$0.10            &  0.70              & $-$0.20           &$-$0.05           &   0.40             &    0.00      &  Marino et al.\,(2011)  \\ %
NGC\,6681 & $-$0.30            &  1.05              & $-$0.85           &   0.00           &   0.20             &    0.00      &    \\ %
NGC\,6715 & $-$0.15            &  0.75              & $-$0.20           &$-$0.10           &   0.50             &    0.05      &    \\ %
NGC\,6717 & $-$0.20            &  0.80              & $-$0.25           &   0.00           &   0.00             &    0.00      &   -- \\ %
          & $-$0.20            &  0.80              & $-$0.10           &$-$0.10           &   0.80             &    0.05      &   -- \\ %
NGC\,6723 & $-$0.35            &  0.80              & $-$0.30           &   0.00           &   0.00             &    0.00      &   -- \\ %
          & $-$0.30            &  0.75              & $-$0.20           &$-$0.10           &   0.80             &    0.05      &   -- \\ %
NGC\,6752 & $-$0.10            &  0.95              & $-$0.40           &$-$0.05           &   0.80             &    0.05      &  Yong et al.\,(2005)  \\ %
NGC\,6779 & $-$0.35            &  1.10              & $-$1.00           &   0.00           &   0.00             &    0.00      &   -- \\
          & $-$0.30            &  0.95              & $-$0.60           &$-$0.10           &   0.80             &    0.05      &   -- \\ %
NGC\,6809 & $-$0.05            &  0.80              & $-$0.20           &   0.00           &   0.50             &    0.00      &    \\ %
NGC\,6838 & $-$0.40            &  0.60              & $-$0.25           &   0.00           &   0.00             &    0.00      &  M{\'e}sz{\'a}ros et al.(2015)  \\ %
NGC\,6934 & $-$0.40            &  0.90              & $-$0.65           &   0.00           &   0.00             &    0.00      &   -- \\
          & $-$0.30            &  0.85              & $-$0.35           &$-$0.10           &   0.80             &    0.05      &   -- \\ %
NGC\,6981 & $-$0.15            &  0.80              & $-$0.35           &   0.00           &   0.00             &    0.00      &   -- \\
          & $-$0.10            &  0.75              & $-$0.10           &$-$0.10           &   0.80             &    0.05      &   -- \\ %
NGC\,7078 & $-$0.20            &  0.85              & $-$0.50           &$-$0.20           &   0.50             &    0.10      &    \\ %
NGC\,7089 & $-$0.35            &  0.70              & $-$0.60           &$-$0.10           &   0.40             &    0.00      &    \\
NGC\,7099 &    0.00            &  0.80              & $-$0.40           &   0.00           &   0.30             &    0.00      &    \\ %
\hline
\hline
          &                     &                   &2Ge-1Ge            &                  &                    &              & \\
\hline   
 IC\,4499 & $-$0.10            &  0.85              & $-$0.60           &   0.00           &   0.00             &    0.00      &  --  \\
          & $-$0.05            &  0.55              & $-$0.00           &$-$0.30           &   1.10             &    0.10      &  --  \\
NGC\,104  & $-$0.55            &  0.90              & $-$0.50           &                  &                    &              &    \\
NGC\,288  & $-$0.20            &  0.75              & $-$0.75           &   0.00           &                    &    0.00      &    \\
NGC\,362  & $-$0.40            &  0.95              & $-$0.65           &$-$0.10           &   0.50             &    0.05      &    \\
NGC\,1261 & $-$0.40            &  1.00              & $-$0.75           &   0.00           &   0.00             &    0.00      &    \\
          & $-$0.45            &  0.85              & $-$0.75           &$-$0.30           &   1.10             &    0.10      &    \\
NGC\,1851 & $-$0.35            &  1.12              & $-$0.55           &$-$0.05           &   1.00             &    0.05      &    \\
NGC\,2298 & $-$0.40            &  1.05              & $-$1.50           &   0.00           &   0.00             &    0.00      &    \\
          & $-$0.45            &  0.85              & $-$0.85           &$-$0.30           &   1.10             &    0.10      &    \\
NGC\,3201 & $-$0.45            &  1.10              & $-$1.10           &   0.00           &   0.90             &    0.00      &    \\ %
NGC\,4590 & $-$0.20            &  0.90              & $-$0.60           &   0.00           &   0.40             &    0.00      &    \\ %
NGC\,4833 & $-$0.15            &  1.05              & $-$0.70           &$-$0.40           &   0.80             &    0.10      &    \\ %
NGC\,5024 & $-$0.30            &  0.75              & $-$1.25           &$-$0.10           &   1.00             &    0.00      &    \\ %
NGC\,5053 & $-$0.00            &  0.70              & $-$0.40           &$-$0.10           &   1.00             &    0.10      &    \\ %
NGC\,5272 & $-$0.30            &  0.85              & $-$0.65           &$-$0.30           &   0.90             &    0.15      &  Sneden et al.\,(2004)  \\ %
NGC\,5286 & $-$0.60            &  1.20              & $-$1.50           &   0.00           &   0.00             &    0.00      &    \\ %
          & $-$0.60            &  0.95              & $-$0.90           &$-$0.30           &   1.10             &    0.10      &    \\ %
NGC\,5466 & $-$0.05            &  0.50              & $-$0.30           &   0.00           &   0.70             &    0.00      &    \\ %
NGC\,5904 & $-$0.45            &  1.10              & $-$0.80           &$-$0.10           &   1.10             &    0.10      &    \\ %
NGC\,5927 & $-$0.80            &  0.35              & $-$0.50           &   0.00           &   0.20             &    0.00      &  Pancino et al.\,(2017)  \\ %
NGC\,5986 & $-$0.50            &  1.10              & $-$0.90           &$-$0.40           &   1.10             &    0.05      &    \\ %
NGC\,6093 & $-$0.15            &  1.15              & $-$0.65           &$-$0.10           &   1.00             &    0.00      &    \\ %
NGC\,6101 & $-$0.30            &  0.90              & $-$0.65           &   0.00           &   0.00             &    0.00      &    \\ %
          & $-$0.30            &  0.65              & $-$0.05           &$-$0.30           &   1.10             &    0.10      &    \\ %
NGC\,6121 & $-$0.15            &  0.80              & $-$0.20           &   0.00           &   0.05             &    0.00      &  Marino et al.\,(2008)  \\ %
NGC\,6144 & $-$0.10            &  0.85              & $-$0.55           &   0.00           &   0.00             &    0.00      &    \\ %
          & $-$0.10            &  0.65              &    0.00           &$-$0.30           &   1.10             &    0.10      &    \\ %
NGC\,6171 & $-$0.30            &  0.70              & $-$0.30           &   0.00           &   0.00             &    0.00      &  M{\'e}sz{\'a}ros et al.(2015)  \\ %
NGC\,6205 & $-$0.25            &  1.10              & $-$0.90           &$-$0.30           &   1.10             &    0.00      &    \\ %
NGC\,6218 & $-$0.35            &  0.95              & $-$0.60           &   0.00           &   0.50             &    0.00      &    \\ %
NGC\,6254 & $-$0.55            &  1.10              & $-$1.05           &$-$0.20           &   1.00             &    0.00      &    \\ %
NGC\,6304 & $-$0.80            &  0.65              & $-$0.45           &   0.00           &   0.00             &    0.00      &  --  \\ %
          & $-$0.95            &  0.60              & $-$0.50           &$-$0.30           &   1.10             &    0.10      &  --  \\ %
NGC\,6341 & $-$0.50            &  0.85              & $-$0.50           &$-$0.40           &   1.30             &    0.00      &    \\ %
NGC\,6352 & $-$0.60            &  0.70              & $-$0.35           &   0.00           &   0.00             &    0.00      &  --  \\ %
          & $-$0.75            &  0.60              & $-$0.35           &$-$0.30           &   1.10             &    0.10      &  --  \\ %
NGC\,6362 & $-$0.55            &  0.75              & $-$0.70           &$-$0.00           &   0.00             &    0.00      & Massari et al.\,(2017)   \\ %
NGC\,6366 & $-$0.60            &  0.70              & $-$0.30           &$-$0.10           &   0.20             &    0.10      & Johnson et al.\,(2016); Puls et al.\,(2018)   \\ %
NGC\,6388 & $-$0.40            &  0.70              & $-$0.15           &$-$0.05           &   0.40             &    0.05      & Carretta \& Bragaglia (2018)   \\ %
NGC\,6397 & $-$0.20            &  0.75              & $-$0.30           &   0.00           &   0.00             &    0.00      &    \\ %
NGC\,6441 & $-$1.05            &  0.85              & $-$0.50           &   0.25           &   0.50             &    0.20      &  Gratton et al.\,(2006); Carretta et al.\,(2009)  \\ %
NGC\,6496 & $-$0.45            &  0.50              & $-$0.25           &   0.00           &   0.00             &    0.00      &  --  \\ %
          & $-$0.60            &  0.40              & $-$0.25           &$-$0.30           &   1.10             &    0.10      &  --  \\ %
NGC\,6535 & $-$0.15            &  0.75              & $-$0.40           &   0.00           &   0.40             &    0.00      &    \\ %
NGC\,6541 & $-$0.50            &  1.30              & $-$1.40           &   0.00           &   0.00             &    0.00      &  --  \\ %
          & $-$0.40            &  1.05              & $-$0.75           &$-$0.30           &   1.10             &    0.10      &  --  \\ %
NGC\,6584 & $-$0.10            &  0.85              & $-$0.35           &   0.00           &   0.00             &    0.00      &  --  \\ %
          & $-$0.10            &  0.60              &    0.10           &$-$0.30           &   1.10             &    0.10      &  --  \\ %
NGC\,6624 & $-$0.70            &  0.70              & $-$0.55           &   0.00           &   0.00             &    0.00      &  --  \\
          & $-$0.85            &  0.60              & $-$0.60           &$-$0.30           &   1.10             &    0.10      &  --  \\
NGC\,6637 & $-$0.45            &  0.75              & $-$0.40           &   0.00           &   0.00             &    0.00      &  --  \\
          & $-$0.60            &  0.70              & $-$0.40           &$-$0.30           &   1.10             &    0.10      &  --  \\
NGC\,6652 & $-$0.45            &  0.75              & $-$0.30           &   0.00           &   0.00             &    0.00      &  --  \\ %
          & $-$0.50            &  0.65              & $-$0.50           &$-$0.30           &   1.10             &    0.10      &  --  \\ %
NGC\,6656 & $-$0.35            &  0.95              & $-$0.55           &$-$0.10           &   0.70             &    0.10      &  Marino et al.\,(2011)  \\ %
NGC\,6681 & $-$0.30            &  1.25              & $-$1.10           &$-$0.10           &   0.60             &    0.00      &    \\ %
NGC\,6715 & $-$0.45            &  1.05              & $-$1.10           &$-$0.40           &   1.20             &    0.10      &    \\ %
NGC\,6717 & $-$0.40            &  0.95              & $-$0.40           &   0.00           &   0.00             &    0.00      &   -- \\
          & $-$0.40            &  0.80              & $-$0.15           &$-$0.30           &   1.10             &    0.10      &   -- \\
NGC\,6723 & $-$0.80            &  1.05              & $-$0.95           &   0.00           &   0.00             &    0.00      &   -- \\
          & $-$0.85            &  0.95              & $-$0.80           &$-$0.30           &   1.10             &    0.10      &   -- \\
NGC\,6752 & $-$0.40            &  1.25              & $-$0.80           &$-$0.25           &   1.10             &    0.10      &  Yong et al.\,(2005)  \\ %
NGC\,6779 & $-$0.50            &  1.40              & $-$1.50           &   0.00           &   0.00             &    0.00      &   -- \\
          & $-$0.45            &  1.10              & $-$0.80           &$-$0.30           &   1.10             &    0.10      &   -- \\
NGC\,6809 & $-$0.20            &  1.10              & $-$0.70           &$-$0.10           &   1.00             &    0.00      &    \\ %
NGC\,6838 & $-$0.45            &  0.60              & $-$0.40           &   0.00           &   0.00             &    0.00      &  M{\'e}sz{\'a}ros et al.(2015)  \\ %
NGC\,6934 & $-$0.50            &  1.10              & $-$0.90           &   0.00           &   0.00             &    0.00      &   -- \\
          & $-$0.50            &  0.85              & $-$0.35           &$-$0.30           &   1.10             &    0.10      &   -- \\
NGC\,6981 & $-$0.60            &  1.15              & $-$1.50           &   0.00           &   0.00             &    0.00      &   -- \\
          & $-$0.60            &  0.90              & $-$0.90           &$-$0.30           &   1.10             &    0.10      &   -- \\
NGC\,7078 & $-$0.50            &  1.00              & $-$0.80           &$-$0.50           &   1.10             &    0.30      &    \\ %
NGC\,7089 & $-$0.65            &  0.75              & $-$1.20           &$-$0.40           &   1.10             &    0.10      &    \\
NGC\,7099 & $-$0.15            &  1.00              & $-$0.80           &   0.00           &   0.50             &    0.00      &    \\ %
\hline
\end{longtable}
% 5139 2808

